MeTeoR: Practical Reasoning in Datalog with Metric Temporal Operators

DatalogMTL is an extension of Datalog with operators from metric temporal logic which has received significant attention in recent years. It is a highly expressive knowledge representation language that is well-suited for applications in temporal ontology-based query answering and stream processing. Reasoning in DatalogMTL is, however, of high computational complexity, making implementation challenging and hindering its adoption in applications. In this paper, we present a novel approach for practical reasoning in DatalogMTL which combines materialisation (a.k.a. forward chaining) with automata-based techniques. We have implemented this approach in a reasoner called MeTeoR and evaluated its performance using a temporal extension of the Lehigh University Benchmark and a benchmark based on real-world meteorological data. Our experiments show that MeTeoR is a scalable system which enables reasoning over complex temporal rules and datasets involving tens of millions of temporal facts.

==> back.tex <==
whether before going to the automata based approach, we perform partial materialisation by setting a threshold (which in the current implementation is fixed and set to the number of rules in $\Prog$) on the number of rounds of rule application; this allows us to construct a part of the least model. If this is not sufficient to verify whether $\Prog$ and  $\mathcal{D}$ entail  $M@\varrho$, then we use the constructed \emph{partial materialisation} to exploit the automata-based technique. The advantage of our approach is that it is suitable for arbitrary programs (unlike pure materialisation), but tries to avoid a computationally challenging construction of automata (unlike the pure automata-based approach).

An additional benefit of our approach is that  the partial materialisation we construct is independent of the fact whose entailment we check. Once constructed, the partial materialisation is kept in memory and can be used for checking entailment of any other fact. This has a clear practical advantage in a reasonable setting where program and dataset do not change frequently.

A program $\Prog$ could possibly consists of dozens or hundreds of rules, but for a given fact, checking its  entailment may not need to involve all rules in $\Prog$. From the point view of operational efficiency, it is a wise option to only involve rules directly or indirectly depended on by the target fact for both materialisation and automata based approaches. To this end, we build a dependency directed graph for $\Prog$, denoted as $G$, in which the node is the predicate and each predicate in the body of a rule points to the head predicate of the rule.

After constructing the dependency graph, we first apply Tarjan's algorithm~\cite{tarjan1972depth} to find all strongly connected components, and each component with more than one predicate are considered as a cycle in which rules involved in the cycle are recursive rules. In particular, for a rule like $\boxplus_{1year} \mathit{Birthday(x)} \gets  \mathit{Birthday(x)}$, we consider as different nodes two predicates appearing in the head and in the body of a rule, respectively, even they have the same name. After finding all strongly connected components, we treat each component as a individual node to form a new dependency graph, denoted as $G'$. We then utilize the topological sorting algorithm~\cite{kahn1962topological} to sort all nodes in $G'$  such that for every directed edge $ab$ from vertex a to vertex b, b comes before a in the ordering.

\smallskip

\noindent \textbf{Calculate $\Prog^{M}$.}  For a given program $\Prog$ and a fact $M@\varrho$, involving all rules in $\Prog$ is an inefficient option, so we propose a dependency graph based technique for identifying a (typically small) subset of of rules that is sufficient for verifying the entailment of the given fact. To be more specific, we hope to only include those rules directly or indirectly depended on by $M$ in order to optimize the operational efficiency. The calculation $\Prog^{M}$ goes as follows: First, based on the topological sorting result on $G'$, we locate the node in which the predicate $M$ is included, denoted as $N_{M}$ and then we select all nodes ahead of $N_{M}$, whose associated rules are regarded as $\Prog^{M}$.  For instance, if the predicate of the fact needed to be entailed is $E$ shown in Figure~\ref{fig:graph}, then we can obtain $\Prog^{E}$ according to the topological sorting result in $\textbf{G'}$.

\smallskip

\noindent \textbf{Temporal fact generation.} Having both a dataset $\D$ and a DatalogMTL program $\Pi$, we then need to generate some temporal facts used for the entailment checking task.  To be more specific,  each temporal fact ready for the entailment checking is in the form of $M@\varrho$, in which $M$ is a ground relational atom randomly selected from the given dataset and $\varrho$ is randomly selected interval. For $\Prog_{nr}$ and $\Prog_{nrr}$ programs, the entailment of temporal facts could be verified by \emph{partial materialisations}, namely, by performing a certain number of rounds of rule applications. Besides, to evaluate the feasibility of the automata based approach, we specially design four temporal facts based on $\Prog_{r}$, denoted as $M^{r}_{1}@\varrho$,  $M^{r}_{2}@\varrho$,  $M^{r}_{3}@\varrho$,  $M^{r}_{4}@\varrho$, respectively,  which are not entailed by $\Prog_{r}$ program and any of the datasets, and so, our algorithm has to perform automata construction.

\begin{table}[t]
\begin{align*}
\textit{LecturerCandidate}(x) &\gets \boxminus_{[0,1]}\textit{GraduateStudent}(x),\textit{publicationAuthor}(y,x),\textit{Publication}(y) \\
\textit{LecturerCandidate} (x) &\gets \boxminus_{[0,1]}\textit{TeachingAssistant}(x),\diamondminus_{[0,1]}\textit{publicationAuthor}(y,x), \\
\textit{Expert(x)} & \gets \textit{FullProfessor}(x), \boxminus[0,2]\textit{researchInterest}(x,y) \\
\textit{GoodDepartment}(y) & \gets  \boxminus_{[0,2]}\textit{worksFor}(x,y),\textit{Expert}(x) \\
\textit{SmartStudent}(x) & \gets \textit{memberOf}(x,y), \textit{GoodDepartment}(y) \\
\textit{SmartStudent}(x) & \gets  \textit{memberOf}(x,y), \textit{GoodDepartment}(y)\\
\textit{SmartStudent}(x) & \gets \textit{memberOf}(x,y), \textit{GoodDepartment}(y) \\
\textit{GoodDepartment}(x) & \gets \boxminus_{[0,4]}\textit{SmartStudent}(x), \diamondminus_{[0,1]}\textit{publicationAuthor}(y,x)\\
\textit{Scientist}(x)& \gets \diamondminus_{[1,2]}\textit{FullProfessor}(x) \\
\textit{FullProfessor}(x) & \gets  \diamondminus_{[1,2]}\textit{Scientist}(x) \\
\end{align*}
\caption{$10$ manully constructed rules with MTL operators}
\end{table}

$\Prog=\{\textit{AssistantProfessor}(x) \gets \boxminus_{[0,3yrs]}\textit{Lecturer}(x),
\textit{AssociateProfessor}(x)  \gets  \boxminus_{[0,4yrs]}\textit{AssistantProfessor}(x)\}$, $\textit{FullProfessor}(x)   \gets \boxminus_{[0,5yrs]}\textit{AssociateProfessor}(x)\}$.


\section{Appendix 1.2}

\subsection{Materialisation-related pseudocodes}
For each rule $r$ in $\Prog$, it is evaluated by Algorithm~\ref{evaluate}, and the derived results are added to $\Delta$. The body of $r$ is represented as $[L_1, \cdots, L_n]$, where $n$  is the
number of metric atoms in the body. Each $L_i$ is variable-free or variable-contained, thus we need to execute the join operation over $[L_1, \cdots, L_n]$ until all metric atoms are variable-free. $L_i\sigma$ denotes a variable-free literal in which all variables in $L_i$ are substituted with constants in $\sigma$, where $\sigma$ is a variable-to-constant mapping dictionary.

It is obvious that multiple successful substitution results exist, so for each substitution result, denoted as $[L_1\sigma, \cdots, L_n\sigma]$, we will apply \emph{ApplyOperator} to $L_i\sigma$, and get the corresponding set of intervals, $T_i$. Having $[T_1, \cdots, T_n]$, we need to get the final set of intervals which are the intersection of $[T_1, \cdots, T_n]$, and the pseudocode for the merging process is shown in Algorithm~\ref{IntervalMerge}.

\SetKwRepeat{DoWhile}{do}{while}
\begin{algorithm}
       \SetKwInput{Input}{Input}
       \SetKwInput{Output}{Output}
       \Input{$\D, \Prog,  K$}
       \Output{$\D$ saturated with all facts by materialisation}
       $k=0$\\
       \DoWhile{$\Delta \neq \emptyset$ and $k<K$}{
           $k=k+1$ \\
           $\Delta \coloneqq \emptyset$ \\
           \For{each rule $r$ in $\Prog$}{
               $\Delta \coloneqq \Delta \cup  \mathsf{Evaluate}(\D, r)$
           }
           $\Delta \coloneqq \Delta \setminus \D$ \\
           $\D \coloneqq \D \cup \Delta$\\
      }
      \KwRet $\D$
  \caption{Materialise}\label{materialisation}
\end{algorithm}

\begin{algorithm}

     \SetKwInput{Input}{Input}
     \SetKwInput{Output}{Output}
     \Input{$\D, r$}
     \Output{a list of list of Intervals, $H$}

     Order the body of $r$ as $L_1, ..., L_n$ \\
     $\sigma \gets \{\}$  \\
     $i \coloneqq 1$, \quad $H \coloneqq \emptyset$ \\
     \While{$i > 0$}{
         Find the next substitution for $L_i \sigma$ and modify $\sigma$ \\
         \If{the substitution is found}{
             \If{$i < n$}{
                 $i \gets i + 1$
             }
             \Else{
                 $T_1 \coloneqq \dots \coloneqq T_n \coloneqq \emptyset$ \\
                 \For{each $L_i\sigma$ with $1 \leq i \leq n$}{
                      $T_i$ $\coloneqq$ $\mathsf{ApplyOperator}(L_i\sigma, \D)$
                   }
                   $T$ $\coloneqq$ $\mathsf{IntervalMerge}([T_1, \dots, T_n]$) \\
                   \For{each $interval$ in $T$}{
                       \textrm{add $h(r\sigma)@interval$ to $H$}
                   }
             }
         }
         \Else{
             $i \gets i - 1$
         }
     }
     \KwRet $H$
    \caption{Evaluate}\label{evaluate}
\end{algorithm}


\begin{algorithm}
        \SetKwInput{Input}{Input}
        \SetKwInput{Output}{Output}
        \Input{$[T_1, \cdots, T_n]$}
        \Output{a list of Intervals, $I$}


         $I \coloneqq \emptyset$\\
         \For{each $i$ with $\{1 \leq i \leq n\}$}{
            sort $T_i$ based on the left value of each interval in $T_i$ \\
         }
		    $p_1$$ \coloneqq T_1.first(), \cdots, p_n \coloneqq T_n.first()$ \\
        \While{$p_i$ is not null for each $i$ with $1 \leq i \leq n$}{
            $target \coloneqq [p_1.lEnd, p_1.rEnd]$ \\
            \For{each $p_i$ with $1 \leq i \leq n$}{
			          $new \coloneqq null$\\
                \While {$new$ is null and $p_i$ is not null}{
                    $new \coloneqq target \cap [p_i.lEnd, p_i.rEnd]$, $p_i \coloneqq p_i.next()$\\

                }

			      	$target \coloneqq new$

      				\If{$target$ is null}{
      				    $\mathbf{break}$
      				}
          }
          \If{$target$ is not null}{
    			    \For{each $p_i$ with $1 \leq i \leq n$}{
                    \If{$target.rEnd < p_i.rEnd$}{
                        $p_i.lEnd \coloneqq target.rEnd$
                    }
                    \Else{
                        $p_i \coloneqq p_i.next()$
                    }
    			     }
               add $target$ to $I$
           }
         }
        \KwRet $I$
    \caption{MergeInterval}\label{mergeinterval}

\end{algorithm}


\begin{table*}[t]
\begin{center}
\begin{tabular}{ c|c|c|c|c }
\toprule
operation & left endpoint & right endpoint & left-open iff left endpoint is $-\infty$ or & right-open iff right endpoint is  $+\infty$ or
 \\
\midrule
$\varrho_1^c$  & $\varrho_1^-$ &  $\varrho_1^+$ &  never  &  never
\\
$\varrho_1 - \varrho_2$  & $\varrho_1^- - \varrho_2^+$ &  $\varrho_1^+ - \varrho_2^-$  & $\varrho_1$ is left-open or $\varrho_2$ is right-open  &  $\varrho_1$ is right-open or $\varrho_2$ is left-open
\\
$\varrho_1 \ominus \varrho_2$  & $\varrho_1^- - \varrho_2^-$ &  $\varrho_1^+ - \varrho_2^+$  & $\varrho_1$ is left-open and $\varrho_2$ is left-closed  &  $\varrho_1$ is right-open  and $\varrho_2$ is right-closed
\\
$\varrho_1 + \varrho_2$  & $\varrho_1^- + \varrho_2^-$ &  $\varrho_1^+ + \varrho_2^+$  & $\varrho_1$  or $\varrho_2$ is left-open  &  $\varrho_1$  or $\varrho_2$ is right-open
\\
$\varrho_1 \oplus \varrho_2$   & $\varrho_1^- + \varrho_2^+$ &  $\varrho_1^+ + \varrho_2^-$  & $\varrho_1$ is left-open and $\varrho_2$ is right-closed  &  $\varrho_1$ is right-open and $\varrho_2$ is left-closed
\\
\bottomrule
\end{tabular}
\end{center}
\caption{
Operations on intervals, where we assume that $-\infty + x = - \infty$ and $  + \infty + x = + \infty$ for any value $x$.
}
\label{tab:operation}
\end{table*}

$\emph{ApplyOperator}$ is implemented strictly according to the semantics of datalotMTL. Specifically, as described before, in order to cope with both open-interval and close-interval scenario, we define a time point as  a class, which the direction and the bracket as well as the value itself. When executing one of the four operations, the sign of closeness and openness would be considered as well as the values. The operation of $-$, $\ominus$, $+$, $\oplus$ used in Aglorithm~\ref{applyoperator} is shown in Table~\ref{tab:operation}.

\begin{algorithm}

      \SetKwInput{Input}{Input}
      \SetKwInput{Output}{Output}
      \Input{$literal, \D$}
      \Output{a list of Intervals, $T$}

      define an empty list, $T$ \\

      \If{$literal$ is atom}{

          $M$ $\gets$ $\{f_1, f_2, \cdots, f_n\}$, \textrm{where} $f_i$ \textrm{is a literal-matched fact in $\D$}

          \For{each $f$ in $M$}{
                  add f.interval to $T$
          }

          \KwRet $T$
      }

      \Else{

            $O = literal.getOp()$ \\
            \If{$O = \Ui$}{

               $L_l \gets literal.leftLiteral$, $L_r \gets literal.rightLiteral$ \\

               $T_l \gets$ ApplyOperator($L_l, \D$),  $T_l \gets$ ApplyOperator($L_r, \D$) \\

               \For{each $t_l \in T_l$}{
                    \For{each $t_r \in T_r$}{
                        \If{$literal.interval.left\_open$ and $literal.interval.left\_value$  $== 0$}{

                            add $+(t_r, literal.interval)$ to $T$ \\
                        }

                        $s \gets intersection(t_l, t_r)$, $t \gets +(s, literal.interval)$\\

                        $t \gets intersection(t_l, t)$, add $t$ to $T$ \\

                    }

               }


            }
            \ElseIf{$O == \Si$}{

                $L_l \gets literal.leftLiteral$, $L_r \gets literal.rightLiteral$ \\

                $T_l \gets$ ApplyOperator($L_l, \D$),  $T_r \gets$ ApplyOperator($L_r, \D$) \\

                \For{each $t_l \in T_l$}{
                     \For{each $t_r \in T_r$}{
                         \If{$literal.interval.left\_open$ and $literal.interval.left\_value$  $== 0$}{

                             add $-(t_r, literal.interval)$ to $T$ \\
                         }

                         $s \gets intersection(t_l, t_r)$, $t \gets -(s, literal.interval)$\\

                         $t \gets intersection(t_l, t)$, add $t$ to $T$ \\

                     }

                }

            }

            \Else{
                $literal \gets literal.removeOp()$ \\

                $ T_{lr} \gets$ ApplyOperator(literal, $\D$)\\

                \If{$O == \diamondminus$}{
                     \For{each $t \in T_{lr}$}{
                        $interval \gets +(literal.interval, t)$ \\

                        add $interval$ to $T$ \\
                     }

                }
                \ElseIf{$O == \boxminus$}{
                     \For{$each t \in T_{lr}$}{
                        $interval \gets \oplus(literal.interval, t)$ \\

                        add $interval$ to $T$ \\
                     }

                }
                \ElseIf{$O == \diamondplus$}{
                     \For{each $t \in T_{lr}$}{
                        $interval \gets  -(literal.interval, t)$ \\

                        add $interval$ to $T$ \\
                     }

                }
                \ElseIf{$O == \boxplus$}{
                     \For{each $t \in T_{lr}$}{
                        $interval \gets \ominus(literal.interval, t)$ \\

                        add $interval$ to $T$ \\
                     }

                }

                \KwRet $T$

          }

      }
      \caption{ApplyOperator}\label{applyoperator}
\end{algorithm}

\subsection{Automata-related pseudocodes}

\input{optimization}

Firstly, we denote with $mat(\Prog, D)$ the powerset of ground literals consisting of $\Top$, all groundings of literal in $\Prog$ by constants in $\Prog$ and $D$, and literals $\boxminus_{[0,\infty)}\alpha$, $\boxminus_{(0,\infty)}\alpha$, $\boxplus_{[0,\infty)}\alpha$ and $\boxplus_{(0,\infty)}\alpha$ for $\alpha$ an atom in $D$. For example, if $D=\{A\}$ and $\Prog = \{\diamondminus_{[1,2]}A\}$, $mat(\Prog, D)$ contains: $\{\}$, $\{A\}$, $\{\diamondminus_{[1,2]}A\}$, $\{\boxminus_{[0,\infty)}A\}$, $\{A, \diamondminus_{[1,2]}A\}$, etc. The size of $mat(\Prog, D)$ would be $2^{6} = 81$.

Secondly, we need to determine the size of window required for the automata. In our setting, we define the targeted window interval as $Q = [-x-z, x+z]$, where $x$ is the biggest rational number in $\D$ and $z$ is the biggest rational number in all intervals of temporal operations in $\Prog$.

Thirdly, directly determining a valid window from the interval $Q$ is non-trivial and inefficient. According to \cite{walega2019datalogmtl}, it is feasible to start from a minimal length of a window($2z$), so we choose $l_{min}=[-x-z, -x+z]$ as our initial window interval.

Fourthly, the most tough part is what literals and atoms should be installed at each ruler interval. If we adopt the brute force method, namely, enumerating the power set of $mat(\D, \Prog)$ from scratch, the search space is extremely huge. Therefore, we consider some tricks, which can potentially speed up the discovery of a valid model.\footnote{It is effective only when there exists a model in which the given query holds.} Given a initial window $W$, consisting of a certain number of ruler intervals, we then conclude our installation tricks as follows:
\begin{itemize}
    \item To avoid some unnecessary search work, our program will first run the materialization until there are no new facts generated in the given interval, $[-x-z, x+z]$, and intermediate results are stored, which can help us determine some must-installed literals or atoms in each ruler interval of the window. After the materialization, for each  ruler interval in $W$, if it is in the range $[-x-z, x+z]$, the corresponding atoms and literals are installed in advance, which can greatly reduce the number of different combinations while keeping the correctness.

    \item For each $\boxplus$ unbounded literal, we take each ruler interval as a starting point, and we find that from that point onward to the most right border of
    $Q$, x+z, the corresponding atom should always be installed, then we will preferentially put the unbounded literal in the chosen ruler interval and its subsequent ruler intervals. Similar for those $\boxminus$ unbounded literals.

    \item According to our experiment, we observe that for those uncertain literals or atoms, it can speed up the discovery of a valid if we preferentially choose not to install them at first, namely, we iterate the combination of  the rest of atoms and literals from $null$ to $all$.

\end{itemize}

Next, we describe how to find a valid target window, whose interval is $Q =[-x-z, x+z]$.
Starting from the initial window interval $l_{min}=[-x-z, -x+z]$, we install some literals and atoms at each ruler of $l_{min}$ according to our strategies. If it is checked to be satisfied according to our \emph{CheckSatisfiability}, then it will move right one ruler-interval while the most left ruler interval will be removed. Applied the same installation strategies to the most right newly-added  ruler interval, and then the new window's satisfiability is checked using \emph{CheckSatisfiability}. The process is repeated until the window reaches to the right endpoint of $Q$, namely, $x+z$.

Having the valid window, $W$, whose range is $[-x-z, x+z]$, we then are ready to define the two automata that we use for consistency checking. The automata is parametrised by a window $W$, which determines the initial state. We take the most left interval~($[-x-z, -x+z]$ of $W$, denoted as $W_{lmin}$ and the most right interval~($[x-z, x+z$) of $W$, denoted as $W_{rmin}$.

\emph{Search} and \emph{Propagate} are utilized to jointly find a loop that satisfies accepting conditions.


\begin{algorithm}

      \SetKwInput{Input}{Input}
      \SetKwInput{Output}{Output}
      \Input{$\D^{new}, \Prog^{new}, x, z, \D$}
      \Output{$true$ or $false$}

       \If{$\bot \notin $ heads of~ $\Prog$ }{
          \KwRet  $true$
       }

       Materialise($\Prog^{new}, \D, \infty, [-x-z,x+z])$\\
       \If{$\bot$ is derived}{
          \KwRet $false$
        }


        Let $mat(\D^{new}, \Prog^{new})$ be the power set of all ground atoms and literals given $\D^{new}, \Prog^{new}$\\

        $Q = [-x-z, x+z]$ \\

        $l_{min}=[-x-z, -x+z]$\\

        $\mathcal{F}_{l} \coloneqq$ accepting conditions in the left direction\\

        $\mathcal{F}_{r} \coloneqq$ accepting conditions in the right direction\\

        $W^{must} \coloneqq  \{L@ri \in \D \mid ri$  is a ruler interval in $l_{min} \}$\\
        $V \coloneqq \{L@ri \mid L \in mat(\Prog^{new}, \D^{new})$ and $ri$ is a ruler interval in $l_{min}$ and $L@ri \notin \mathsf{D} \}$ \\

        \For{each $W \subseteq V$}{
              $W \coloneqq W \cup W^{must}$

              \If{$CheckSatisfiability(W, \D^{new}, \Prog^{new})$}{

                  $flag, W' \coloneqq SearchWindow(W, \delta_{r}, \D^{new}, \Prog^{new}, \D)$ \\

                  \If{flag}{
                     $W_{lmin} \coloneqq W'.getLeftMinWindow()$ \\
                     $W_{rmin} \coloneqq W'.getRightMinWindow()$ \\

                     \If{Search($W_{lmin}, \delta_{l}, \mathcal{F}_{l}, \D^{new}, \Prog^{new}, \D$)}
                     {
                         \If{Search($W_{rmin}, \delta_{r}, \mathcal{F}_{r}, \D^{new}, \Prog^{new}, \D$)}{
                             \KwRet  $false$
                          }
                     }



                  }
              }


        }
      \KwRet $true$

     \caption{Conistency checking based on the automata approach}
\end{algorithm}

\begin{algorithm}
    \SetKwInput{Input}{Input}
    \SetKwInput{Output}{Output}
    \Input{$W, \delta, \D^{new}, \Pi^{new}, \D$}
    \Output{$true$ or $false$}


     \If{$W$ reaches to $x+z$}
     {
        \KwRet $true, W$
     }

     $r_{r}^{next} \coloneqq$ getNextRInterval($W$) \\

     \For{each $\sigma \subseteq Com(\D^{new}, \Prog^{new}, \D', r_{r}^{next})$}{

           $W = \delta(W, \sigma)$ \\

           \If{CheckSatisfiability($W, \D^{new}, \Prog^{new}, \D$)}
           {
               \KwRet SearchWindow($W, \D^{new}, \Prog^{new}$)
           }
      }

      \KwRet $false, W$

     \caption{SearchWindow}
\end{algorithm}

\begin{algorithm}
    \SetKwInput{Input}{Input}
    \SetKwInput{Output}{Output}
    \Input{$W_0, \delta,  \D^{new}, \Prog^{new}, \D, \mathcal{F}$}
    \Output{$true$ or $false$}

     $T \coloneqq \emptyset$, \quad $R \coloneqq \emptyset$ \\

     $T.push(W_0)$ \\

      \While{$T \neq \emptyset$}{
           $W \coloneqq T.top()$ \\
           \While{$T$ is growing}{
               $r_{r}^{next} \coloneqq$ getNextRInterval($W$) \\

               \For{each $\sigma \subseteq Com(\D^{new}, \Prog^{new}, \D', r_{r}^{next})$}{

                 $W' \coloneqq \delta(W, \sigma)$

                 \If{$\mathsf{CheckSatifiability}(W', \D^{new}, \Prog^{new}))$ and $W' \not \in T \cup R$}{
                     $T.push(W')$\\

                     \quad $label[W'] \coloneqq \emptyset$ \\

                     $W \coloneqq W'$

                     break
                 }
             }
          }

         \If{$label[W] \neq \emptyset$ or $\exists F \in \mathcal{F}$ such that $W \in F$}{

             Propagate($\{W\}$, $label[W] \cup \{F \in \mathcal{F} \mid W \in F\}$, $T$, $R$) \\
             \If{$label[W] == \mathcal{F}$}{
                \KwRet $true$ \\
             }
         }
         $R \coloneqq R \cup \{W\}$ \\
         $T.pop()$ \\

      }


     \KwRet $false$

     \caption{Search}
\end{algorithm}

\begin{algorithm}

    \SetKwInput{Input}{Input}
    \Input{$N, P, T, R, \D^{new}, \Prog^{new}, \D$}


    \While{$N \neq \emptyset$}{
        remove an arbitrary $W$ from $N$

        $r_{r}^{next} \coloneqq \mathsf{getNextRInterval}(W)$

        \For{each $\sigma \subseteq \mathsf{Com}( \D^{new}, \Prog^{new}, \D', r_{r}^{next})$}{

            $W' \coloneqq \delta(W, \sigma)$

            \If{CheckSatifiability($W', \D^{new}, \Prog^{new})$ and $W' \in T \cup R$ and $P \not \subseteq label[W']$}{
                $N \coloneqq N \cup \{W'\}$ \\
                $label[W'] \coloneqq label[W'] \cup P$
            }
        }
    }
    \caption{Propagate}
\end{algorithm}


\begin{algorithm}
  \SetKwInput{Input}{Input}
  \SetKwInput{Output}{Output}
  \Input{$W, \Prog^{new}$}
  \Output{$true$ or $false$}


  \For{each $interval$ within $W$}{
         \For{each rule $r \in \Prog^{new}$}{
             $installed\_literals \coloneqq W[interval]$ \\
             Evaluate $r$ using  $installed\_literals$ \\
             \If{$r.body$ exists and $r.head$ does not exist}{
                \KwRet $false$
             }
         }
    }

    \KwRet $true$

    \caption{CheckSatisfyP}

\end{algorithm}

As for \emph{ChecSatisfiablity}, it mainly consists of three parts.
\begin{itemize}
    \item The first part is to check whether each fact in $\D$ has been installed in the current window $W$ if its interval is within in the window interval.
    \item The second part is to check the self-containedness. To this end, we use $G$ to store all atoms and their intervals in $W$. Besides, for each $\boxplus$ or $\boxminus$ literals, we deduce their required atoms, and then store these deduced atoms to $G$. If $W$ has no Since or Until literals, then we do not need to do the guessing operations. At each ruler interval, we check each literal, $l$, in $\Pi$, namely, we apply \emph{ApplyOperator} to  $l$ and $G$, whose output is $T$. If $T$ is null, then $l$ should not appear in any ruler interval. Otherwise, all ruler interval within in $T$ should contain $l$.  As for the scenario in which since and until literals exist, we will need do the guessing operation, and the guessing results would be added to $G$, and then check all literals in $\Prog$ as before.

    \item In third part, we will enumerate all rule in $\Prog$. For each ruler interval, if all literals in the body exist, then the head should also be installed, otherwise it is not satisfied.

\end{itemize}


\begin{algorithm}

    \SetKwInput{Input}{Input}
    \SetKwInput{Output}{Output}
    \Input{$W, \D^{new}, \Prog^{new}$}
    \Output{$true$ or $false$}


     \For{each ruler interval within $W$}{
          \For{each $literal@interval \in \D^{new}$}{
              \If{$literal@interval \notin W$}{
                   \KwRet $false$ \\
              }
           }
     }

     $G \coloneqq \emptyset$, \quad $B \coloneqq \emptyset$ \\
     \For{each $literal@interval \in W$}{
         \If{$literal$ is an atom}{
            $G[literal] \coloneqq G[literal] \cup \{interval\}$
         }
         \ElseIf{$literal$ is a boxplus literal}{
            Reversely apply boxplus to  $literal@interval$ to obtain $result$\\
            $G[literal.atom] \coloneqq G[literal.atom] \cup \{result\}$
         }
         \ElseIf{$literal$ is a boxminus literal}{
            Reversely apply boxminus to  $literal@interval$ to obtain $result$\\
            $G[literal.atom] \coloneqq G[literal.atom] \cup \{result\}$
         }

         \Else{
             $B \coloneqq B \cup \{literal\}$

         }
     }

     \If{$B \coloneqq \emptyset$}{
        \For{each $literal$ appearing in $\Prog^{new}$}{
            $T \coloneqq \mathsf{ApplyOperator}(literal, G)$ \\
            \If{$T_{\langle W.lEnd, W.rEnd \rangle} \nsucc W$} {
                 \KwRet $false$\\
            }
        }

        \KwRet CheckSatisfyP($W, \Prog^{new}$)
     }



      $LR \coloneqq \emptyset$ \\
      \For{each $A \, o_{\rho} \, \alpha \in B$ where $o$ is either $\Si$ or $\Ui$}{
         add $\alpha$ to $LR$ \\
         \If{$A \neq top$}{
             add $A$ to $LR$
         }
      }

      $GL \coloneqq W.lEnd - z - |LR| * gcd $ \\
      $GR \coloneqq W.rEnd + z + |LR| * gcd$ \\
      $GP \coloneqq [GL, GL+gcd, \cdots, GR]$ \\

      \For{each $G^{'} = \{L_1@i_1, \dots, L_{|LR|}@i_{|LR|}\}$ where $L_k$ is the $k$th element of $LR$ and $i_k$ has both ends in $GP$}{
           $G_{new} \coloneqq G \cup G^{'}$ \\
           \For{each $literal$ appearing in $\Prog^{new}$ }{
              $T \coloneqq$ $\mathsf{ApplyOperator}(literal, G_{new})$ \\
              \If{$T_{\langle W.lEnd, W.rEnd \rangle} \nsucc W$} {
                   \KwRet $false$ \\
              }

          }
      }

     \KwRet CheckSatisfyP($W, \Prog^{new})$

     \caption{CheckSatisfiability}

\end{algorithm}


==> datagenerator.tex <==
\begin{algorithm}[t]
   \SetKwInput{Input}{Input}
   \SetKwInput{Output}{Output}
   \SetKwInput{Parameters}{Parameters}
   \Input{$\hat{\D}$, a set of time-free facts }
   \Parameters{$V_l, V_r$, which confine each randomly-generated interval $\varrho$ to be within $[V_l, V_r]$; $\varphi$, denotes the maximal number of intervals a fact can have.}
   \Output{A dataset $\D$ consisting of temporal facts}
  
   $\D \coloneqq \{\}$ 
    
   \For{each time-free fact $M \in \hat{\D}$}{
       \If{the predicate of $M \in P_1 $}{
           
            randomly generate a list of intervals $T \coloneqq [\varrho_1]$, where $V_l \leq \varrho_1^{-} \leq V_r$ and $\varrho_1^{+} = +\infty$
       
       }
       \ElseIf{the predicate of $M \in P_2$}{
           randomly pick a positive number $n$, $1\leq k \leq \varphi $
           
           randomly generate intervals $T \coloneqq [\varrho_1, \varrho_2, \cdots, \varrho_n]$, where $V_l \leq \varrho_i^{-} \leq V_r$ and $\varrho_i^{+} = \infty$
       }
       \Else{
          randomly select a positive number $n$, $1\geq k \leq \varphi $
           
          randomly generate intervals $T \coloneqq [\varrho_1, \varrho_2, \cdots, \varrho_n]$, where $\varrho_i^{+} \leq \varrho_j^{-}, i < j$, and $\varrho_1^{-} \geq V_l, \varrho_n^{+} \leq V_r$
        }
       
        associate $M$ with each $\varrho_{i} \in T$ to have $ G =\{M@\varrho_1, f@\varrho_2, \cdots, M@\varrho_n$\\
       
        $\D := \D \cup G$\\
       
   }
   \KwRet $\D$
 \caption{Generating temporal datasets}
 \label{algo:gen}
\end{algorithm}

==> datalogmtl.tex <==
\section{DatalogMTL}
We recapitulate the definition of DatalogMTL.
We focus on the rational timeline and the
continuous semantics \cite{walega2019datalogmtl}, as opposed to the
integer timeline \cite{DBLP:conf/ijcai/WalegaGKK20} or the alternative
pointwise semantics \cite{ryzhikov2019data}.

\smallskip

\noindent\textbf{Syntax. }
A \emph{relational atom} is a standard first-order atom of the form $P(\sbf)$, with $P$ a predicate and $\boldsymbol{s}$ a tuple of constants and variables;
it is \emph{ground} if it contains no constants.
A \emph{fact} is an expression  $\matA @ \varrho$
with $\matA$ a ground relational atom and $\varrho$ a rational interval; whereas  a
 \emph{dataset} is a finite set of facts.
A \emph{metric atom} is an expression
given by the following
grammar, where $P(\sbf)$ is a relational atom, while
$\diamondminus$, $\diamondplus$, $\boxminus$, $\boxplus$, $\Si$,  $\Ui$ are MTL operators  indexed with arbitrary rational intervals $\varrho$:
\begin{multline*}
	M  \Coloneqq
		\top  \mid  \bot  \mid
	P(\sbf)  \mid
	\diamondminus_\varrho M   \mid
	\diamondplus_\varrho M   \mid   \\
	\boxminus_\varrho M   \mid
	\boxplus_\varrho M  \mid
	M \Si_\varrho M   \mid
	M \Ui_\varrho M.
\end{multline*}

A  \emph{rule} is an expression of the form
%\begin{align*}
$	\matA'  \leftarrow \matA_1 \land \dots \land \matA_n$, for $n \geq 1$,
%\end{align*}
where each $\matA_i$ is a metric atom, whereas $\matA'$ is a metric atom not mentioning operators $\diamondminus$, $\diamondplus$, $\Si$, and $\Ui$; metric atom  $\matA'$ is the rule's \emph{head}
and the conjunction $\matA_1 \land \dots \land \matA_n$ is its \emph{body}.
A DatalogMTL \emph{program} is a finite set of safe rules---where each variable occurring in the head of a rule occurs also in the body of this rule.

\smallskip

\noindent \textbf{Semantics. }
A DatalogMTL \emph{interpretation} $\I$ specifies, for each ground relational atom $M$ and each time point $t \in \mathbb Q$, whether $M$
holds at $t$, in which case we write ${\mathfrak{I},t \models M}$.
This  extends to metric atoms with MTL operators as follows:
\begin{alignat*}{3}
	&\I, t \models  \top    && && \text{for each } t
	\\
	&\I, t  \models \bot   && && \text{for no } t
	\\
	&\I,  t  \models \diamondminus_\varrho M    && \text{iff}   && \I, t' \models  M \text{ for some } t' \text{ with } t -   t' \in \varrho
	\\
	&\I,  t  \models  \diamondplus_\varrho  M  && \text{iff} &&  \I,  t' \models    M  \text{ for some } t'  \text{ with } t' - t \in \varrho
	\\
	&\I, t  \models \boxminus_\varrho  M  && \text{iff} && \I, t' \models M \text{ for all } t' \text{ with } t-t' \in \varrho
	\\
	&\I,t  \models \boxplus_\varrho  M   && \text{iff} && \I,t' \models  M \text{ for all } t'  \text{ with } t'-t \in \varrho
	\\
	&\I,t  \models M_1 \Si_\varrho M_2   &&  \text{iff} &&  \I,t' \models  M_2 \text{ for some } t'  \text{ with } t-t' \in \varrho
	\\
	& && && \text{and }  \I,t'' \models  M_1 \text{ for all } t'' \in (t',t)
	\\
	&\I,t  \models  M_1  \Ui_\varrho M_2 \;   &&  \text{iff} \; && \I, t' \models  M_2 \text{ for some } t'  \text{ with } t' - t \in \varrho
	\\
	& && && \text{and }  \I, t'' \models  M_1 \text{ for all } t'' \in (t,t')
\end{alignat*}
An interpretation $\I$ satisfies a metric fact  $\matA @ \varrho$
if $\I,t \models \matA$ for all $t \in \varrho$. An interpretation $\I$ satisfies a ground rule $r$ if, whenever $\I$ satisfies each body atom of $r$ at a time point $t$, then $\I$ also satisfies the head of $r$ at $t$.
An interpretation $\I$ satisfies a (non-ground) rule $r$ if it satisfies each ground  instance of~$r$. An interpretation $\I$ is a \emph{model} of a program $\Prog$ if
it satisfies each rule in $\Prog$, and it is a \emph{model} of a dataset $\D$ if
it satisfies each fact in $\D$.
A program $\Prog$ and a dataset $\D$
are \emph{consistent} if they have a model, and they
\emph{entail} a fact $M@ \varrho$
if each  model of both $\Prog$ and $\D$ is also a model of $M@ \varrho$.


\smallskip

\noindent \textbf{Reasoning. }
The main reasoning tasks in DatalogMTL are \emph{fact entailment}---to check whether a program and a dataset entail a given fact, and \emph{consistency checking}---to check whether a program and a dataset are consistent.
These  problems are polynomially reducible to the complement of each other \cite{brandt2018querying}.

\smallskip


==> images/ablation.tex <==
\begin{figure}[hbt]
 \centering
 \includegraphics[width=0.4\textwidth]{images/bar.png}
 \caption{Results of ablation study}
 \label{fig:ablation}
\end{figure}


==> images/distribution.tex <==
\begin{figure}[hbt]
 \centering
 \includegraphics[width=0.49\textwidth]{images/distribution.png}
 \caption{Distribution of each type over four datasets}
 \label{distribution}
\end{figure}


==> images/graph.tex <==
\begin{figure}[hbt]
 \centering
 \includegraphics[width=0.47\textwidth]{images/graph.png}
 \caption{Dependency graph for the program from Example~\ref{examplegraph}}
 \label{fig:graph}
\end{figure}


==> implementation.tex <==
\section{Implementation Details}
\nb{P: We need to discuss the structure of sections between Preliminaries and Experiments.}
\input{algos/pipeline}
Our implementation focuses on the fact entailment problem.
To check whether a program $\Prog$ and a dataset $\mathcal{D}$ entail a fact $M@\varrho$, we will combine two techniques introduced in the literature: materialisation~\cite{brandt2018querying} and automata construction~\cite{walega2019datalogmtl}.\footnote{For the space limitation,  pseudo-codes for some important algorithms involved in our implementation are provided in Supplementary material.}

\smallskip


\noindent \textbf{Materialisation. }
The first approach is based on the \emph{least model property} of DatalogMTL, which guarantees that whenever $\Prog$ and $\mathcal{D}$ are consistent, they have a unique least model.
%---also called their \emph{materialisation}.
Thus, to check entailment it suffices to verify whether the least model of $\Prog$ and $\mathcal{D}$ satisfies $M@\varrho$.
This model can be constructed by \emph{materialisation} (or forward-chaining)---saturating $\mathcal{D}$ with facts entailed by a `one-step application' of rules in $\Prog$ until a fixpoint is reached, that is, until no new facts can be entailed.
If $\Prog$ is non-recursive, materialisation takes a finite number of steps.
In general, however, materialisation can take a transfinite number of steps, which is in contrast to  Datalog. We give two simple examples to explain the intuition behind the fact that why only involving materialisation is not enough for arbitrary DatalogMTL programs.

\smallskip

\begin{example}
\nb{P: I think this example can be deleted.}
If a program $\Prog_1$ consists of one rule, $ \mathit{Immune(x)} \gets  \boxminus_{[0, 1week]}\mathit{NoSympt(x)}$, stating that individuals without symptoms in the past two weeks are immune. Let now $\D_1$ be a dataset with a single fact $\mathit{NoSympt(James)@[20210401, 20210414]}$, saying that James had no symptoms from the 1st of April 2021 to the 14th of April 2021. The least canonical model of $\Prog_1$ and $\D_1$ could be obtained after one step of rule application, that is, no new fact can be entailed, and the saturated $\D$ would be {$\mathit{NoSympt(James)@[20210401, 20210414]}$, $\mathit{Immune(James)@[20210407, 20210414]}$}.
\end{example}

\smallskip

\begin{example}
\nb{P: I think this example can be deleted.}
Consider, for instance, another program  $\Prog_2$ consisting of  rule $\boxplus_{1year} \mathit{Birthday(x)} \gets  \mathit{Birthday(x)}$, which states that anyone having their birthday at a time point $t$ will also be having their birthday at the same time the following year. Let now  $\D$ be a dataset with a single fact saying that
Alan Turing was having his first birthday during the 23thrd of June 1913. In the canonical model of $\Prog$ and  $\D$, atom $ \mathit{Bday}(\mathsf{Turing})$ holds
at each time within June 23rd  of each year from 1913 onwards, and each step of rule application makes it true on the same day the year after, which denotes that infinitely many rounds of rule application is needed. In this scenario, the materialisation-based approach can not work for checking the entailment of a fact stating Alan Turing's birthday in an infinite future.
\end{example}

\smallskip

\noindent \textbf{Automata. }
\nb{P: This should go to Preliminaries probably.}
For arbitrary DatalogMTL programs another approach has been introduced, where checking entailment of $M@\varrho$ by
$\Prog$ and  $\D$ is reduced to checking inconsistency of a new program $\Prog'$ and dataset $\D'$ which, in turn, is performed by checking emptiness of two B\"{u}chi automata~\cite{walega2019datalogmtl}.
Intuitively, both of the automata have non-empty languages if
there is a model of $\Prog'$ and $\D'$, witnessing their consistency;
otherwise, $\Prog'$ and $\D'$ are inconsistent.

\smallskip

\begin{definition}\label{m-dependent}
Given a fact $M@\varrho$, a rule $r$ is an \emph{$M$-dependent} rule if $M$ in the head of $r$. If $r$ is a \emph{$M$-dependent}\nb{P; I suggest the name "$M$-relevant".} rule, $M'$ is in the body of  $r$ and $M'$ is in the head of of another rule $r'$, then $r'$ is also an \emph{$M$-dependent} rule.
\end{definition}

We are ready to define a dependency graph for a given program $\Prog$.
\begin{definition}\label{graph}
\nb{P: This definition can be much simplified and should probably go to Preliminaries, as this is a well-known dependency graph.}
Let $\Prog$ be a DatalogMTL program and $\Prog'$ be obtained from $\Prog$ in which each rule $r'$ in  $\Prog'$ is obtained from the rule $r$ in $\Prog$ by
removing MTL operators for all metric atoms in both the head and the body of $r$, and then replacing the resulted relation atom $P(s)$ with a proposition $X_{p}$ uniquely associated to $P$.
\end{definition}

The dependency graph of $\Prog$ is a directed multigraph $G_{\Prog}$ with the nodes and the edges given as follows:
\begin{itemize}
    \item[--] A vertex $v_P$ for each proposition $X_P$ in $\Prog'$.
    \item[--] A edge $(v_P, v_Q)$ if there is a rule  $r'$ in $\Prog'$ where $X_Q$ occurs in the head of $r'$ and $X_P$ is in the body of $r'$.
\end{itemize}

\begin{definition}\label{recursive}
A predicate $P$ is recursive if and only if in the dependency graph $G_{\Prog}$, there is proposition $X_Q$\nb{P: You want to talk about vertices, and not propositions here.} which is in a cycle and there is a path from $X_Q$ to $X_P$.
\end{definition}

\begin{definition}\label{non-recursive}
The non-recursive part $\Prog_{non-rec}$ of a program $\Prog$ is a set of rules from $\Prog$ such that all body predicates in these rules are not recursive.
\end{definition}

\input{images/graph}

It is obvious that for the entailment checking of a given fact $M@\varrho$, it is more efficient to only use $\Prog^{M}$ containing $M$-dependent rules instead of involving the whole program $\Prog$, especially when the program $\Prog$ is complicated and the number of rules is large. Besides, we also observe that dividing a program $\Prog$ into $\Prog_{non-rec}$ and $\Prog_{rec}$ is a good optimized option, which can greatly improve the efficiency of our reasoner.  The definition of $\Prog_{non-rec}$ is given in Definition~\ref{non-recursive} and $\Prog_{non-rec} = \Prog \setminus \Prog_{non-rec}$. More specifically, we give an toy example to explain the intuition behind in Example~\ref{examplegraph}.
\begin{example}\label{examplegraph}
In universities, the role change or promotion is a common phenomenon. More specifically, we assume that a lecturer could be directly promoted to be an assistant professor after being in the position for the past continuous three years; similarly, an assistant professor could be directly promoted to be an associate professor after being in the position for the past continuous four years and an associate professor could be directly promoted to be a full professor after being in the position for the past continuous five years; Besides, we assume that roles of a full professor and a chair could be converted if one has ever taken one of the two positions during  the past two years. Finally, we also assume that if a person is the head of an organization and the organization is a department, then the person could be a chair. A DatalogMTL program $\Prog$ representing these dependencies consists of the following rules:
\end{example}
\vspace{-0.4cm}
\begin{align*}
\textit{AssistantProfessor}(x)  & \gets \boxminus_{[0,3yrs]}\textit{Lecturer}(x), \\
\textit{AssociateProfessor}(x)  & \gets  \boxminus_{[0,4yrs]}\textit{AssistantProfessor}(x), \\
\textit{FullProfessor}(x)  & \gets \boxminus_{[0,5yrs]}\textit{AssociateProfessor}(x), \\
\textit{Chair}(x)  &\gets \textit{headOf}(x,y) \land \textit{Department}(y),\\
\textit{FullProfessor}(x)  & \gets \diamondminus_{[0,2yrs]}\textit{Chair}(x), \\
\textit{Chair}(x)  & \gets \diamondminus_{[0,2yrs]}\textit{FullProfessor}(x).
\end{align*}
The dependency graph of this program is given in Figure~\ref{fig:graph}. It has a cycle, which denotes the rules in the cycle are recursive.

Assume the we need to check the entailment of the fact $M@\varrho$ and the predicate of $M@\varrho$ is \emph{AssistantProfessor}, then according to our definition of the $M$-dependent rule in Definition~\ref{m-dependent}, we only have one $M$-dependent rule $\textit{AssistantProfessor}(x)  \gets \boxminus_{[0,3yrs]}\textit{Lecturer}(x)$ for $M@\varrho$. Besides, in Figure~\ref{fig:graph}, according to Definition~\ref{recursive}, we have two recursive predicate, \emph{FullProfessor} and \emph{Chair}. The non-recursive part $\Prog_{non-rec}$  of $\Prog$ contains the first four rules and the rest goes to the recursive part $\Prog_{rec}$.

\smallskip

\noindent \textbf{Pipeline for \emph{fact entailment} checking. }  Algorithm~\ref{alg:pipline} illustrates the whole pipeline for the \emph{fact entailment} checking based on our developed reasoner.

First of all, we get the set of $M$-dependent rules $\Prog^{M}$ for $M@\varrho$. Then, we check whether $\Prog^{M}$ is forward propagating or backward propagating.
\begin{lemma}\label{forwardpropagation}
If $\Prog$ is forward propagating, it means that any time point less than the minimum value of $\D$ can not be reached\nb{P: "cannot be reached" needs reformulation and precise description.};
\end{lemma}
\begin{lemma}\label{backwardpropagation}
If $\Prog$ is backward propagating, any time point larger than the maximum value of $\D$ can not be reached.
\end{lemma}

Thus, if the given $\Prog$ is forward propagating or backward propagating, we can check whether the interval $\varrho$ in $M@\varrho$ is satisfied according to Lemma~\ref{forwardpropagation} and Lemma~\ref{backwardpropagation}, respectively. If $\varrho$ is not satisfied, the checking process is terminated by returning $\mathsf{False}$ representing that the fact $M@\varrho$ is not entailed;

Next, if $\Prog$ is not forward propagating or backward propagating, or $\varrho$ does not violate the propagating properties of $\Prog$, we use  the initial $\D$ to check whether $M@\varrho$ is entailed. If not, we need to involve $\Prog$ to check whether the given $M@\varrho$ is entailed. Given that not all rules in $\Prog$ contribute to the entailment checking, we thus only consider those $M$-dependent rules according to Definition~\ref{m-dependent}, denoted $\Prog^{M}$.

Having $\Prog^{M}$, we first check $\Prog^{M}$ is non-recursive according to Definition~\ref{non-recursive}. If so, we materialise based on $\Prog^{M}$ and $\D$ until $\D \models M@\varrho$ or a fixpoint is reached, that is, no new fact entailed by $\Prog^{M}$ and $\D$ is derived. Once the fixpoint is reached, $\D$, saturated with all facts in the materialisation, provides a representation of the canonical, least model of the input over which all following facts can be directly checked to be entailed or not.

\begin{theorem}\label{bounded}
\nb{P: if $\Prog$ can be unbounded intervals and by "limited number" you mean "finite number", then the statement is false. (Actually, for work with Michał, I am proving now that for bounded $\Prog$ this statement is true.}
If a fact $M@\varrho$ is a bounded fact and meanwhile, is entailed by a given dataset $\D$ and $\Prog$, the entailment of $M@\varrho$ can be verified after a limited number of steps of materialisation.
\end{theorem}

\begin{theorem}\label{inconsistency}
\textcolor{red}{Need to be polished.}To check the inconsistency of a program $\D$ and a dataset $\Prog$, we need to prove that there does not exist a valid model, namely, iterating over all possible combinations to make the conclusion, which has high computational complexity. However, if a fact $M@\varrho$ is not entailed by a given dataset $\D$ and $\Prog$, using the automata based approach is more efficient because we only need to find a valid model to check the consistency.
\end{theorem}

However, if $\Prog^{M}$ is recursive, to check the entailment of a fact $M@\varrho$, there exist following cases,
\begin{itemize}

   \item[case 1] the program $\Prog^{M}$ is finitely materialisable, which means a model can be constructed by \emph{materialisation}(orforward-chaining)—saturating $\D$ with facts entailed by a ‘one-step application’ofrules in $\Prog^{M}$ until a fixpoint is reached, that is, until no new facts can be entailed. In this case, no matter whether $M@\varrho$  is entailed or not entailed, to check entailment it suffices to verify whether the least model of $\Prog^{M}$ and $\D$ satisfies $M@\varrho$;

   \item[case 2] $M@\varrho$ is an entailed fact and no matter whether $\Prog^{M}$ is finitely materialisable or not, it is possible that the entailment of $M@\varrho$ can be verified by a limited number of steps of materialisation;

   \item[case 3] $M@\varrho$ is an non-entailed fact and $\Prog^{M}$ is not finitely materialisable, or $M@\varrho$ is entailed fact but can not be verified by a limited number of steps of materialisation; In either of two case, we need to construct the automata to verify the entailment of $M@\varrho$.

\end{itemize}

To this end, we adopt a paralleled scheme to do the entailment checking, namely, we use two subthreads to run the materialisation and the automata until we confirm the entailment of $M@\varrho$. The intuition behind this is that as described in Theorem~\ref{inconsistency}, it has high computational complexity to use the automata based approach to check the inconsistency of the new dataset $\D'$ and the new program $\Prog'$ when $M@\varrho$ is entailed. However,  according to Theorem~\ref{bounded}, it is feasible and more efficient to use the materialisation based approach to finish the entailment checking task within a limited number of steps of rule application. The reason why we need to use another subthread synchronously to run B\"{u}ichi automata is that if $M@\varrho$ is not entailed, then the materialisation may not stop in \emph{case 3}. We thus need to use the automata based approach to do the consistency checking in order to get a determined entailment result for $M@\varrho$. In particular, it is notorious that the construction of automata is computational challenging, so we propose some optimization tricks to speed up the construction while keeping the correctness. We detail these tricks in the next section.


==> optimization.tex <==
% \section{Optimization for B\"{u}ichi Automata Construction}
%
% \nb{P: I am not sure if we need this section at all?}

Before casting our optimization tricks for B\"{u}chi automata, we first give the definition of windows, which play the role of states in the automata construction.

\begin{definition}
    \label{def::window}
    Let $\varrho$ be an interval with endpoints on the ruler. A \emph{window} over $\varrho$
    is a set $W$ of  generalised facts $M@\varrho'$ with ${M  \in \mathsf{glit}(\Prog, \D)}$ and ruler-intervals $\varrho' \subseteq
    \varrho$ for which there exists a ruler-interpretation $\I$, called \emph{corresponding} to $W$, such that for all ruler-intervals ${\varrho' \subseteq \varrho}$ and $M\in \mathsf{glit}(\Prog, \D)$ we have $\I \models M@ \varrho'$  if and only if  ${M@ \varrho' \in W}$.
\end{definition}

\noindent where, $\mathsf{glit}(\Prog, \D)$  is the set of ground metric atoms consisting of
$\top$, all groundings of metric atoms in $\Prog$ by constants in $\Prog$ and $\D$, and metric atoms $\boxminus_{[ 0, +\infty )} M$, $\boxminus_{( 0, +\infty )} M$, $\boxplus_{[ 0, +\infty )} M$, and $\boxplus_{( 0, +\infty )} M$, for $M$ an atom  in~$\D$; A \emph{ruler} (for $\Prog$ and $\D$) is the set of time points of the form $x +n \cdots \mathsf{gcd}(\Prog)$ for $x$ a rational in $\D$ (or $0$ if $\D = \emptyset$) and $n$ an integer, $\mathsf{gcd}(\Prog)$ is the greatest rational number which divides all rational numbers which are endpoints of intervals  in $\Prog$ to integer values (if $\Pi$ has no numbers, we take $\mathsf{gcd}(\Prog) = 1$ for definiteness).; A \emph{ruler-interval} is either a punctual interval over a time point on the ruler or an interval $(t_1,t_2)$ with $t_1$, $t_2 $ consecutive time points on the ruler. A fragment of the ruler and the corresponding  ruler-intervals for a program $\Prog$ with $\mathsf{gcd}(\Prog)=2.5$ and a dataset $\D = \{ \alpha@[0,0], \beta@[4.2,4.2] \}$ is depicted below,
\input{ruler}


\noindent \textbf{Optimize the selection of the subset of $\mathsf{glit}(\Prog, \D)$}. It is well acknowledge that the size of powerset of $\mathsf{glit}(\Prog, \D)$ increases exponentially with the size of $\Prog$ and $\D$. Obviously, iterating over the whole powerset is unwise and time-consuming. Therefore, given a fact $M@\varrho$, our first optimization trick is to preclude some unnecessary ground metric atoms in $\mathsf{glit}(\Prog, \D)$ to get a new $\mathsf{glit'}(\Prog^{M}, \D^{\Prog^{M}})$, where $\D^{\Prog^{M}}$ denotes part of facts in $\D$ whose predicates appear in $\mathsf{glit'}(\Prog^{M}, \D^{\Prog^{M}})$.

After obtaining the new $\mathsf{glit'}(\Prog^{M}, \D^{\Prog^{M}})$, we divide the ground metric atoms into two sets: one is $A_{variant}$ whose predicates appears in recursive parts of $\Prog^{M}$, and the rest goes to the set $A_{invariant}$. For metric atoms whose predicates in $A_{invariant}$, we can have determined answers about whether they should be included in each ruler interval of the window or not according to results of \emph{partial materialisation}. Besides, another advantage is that we do not need to bind these $\boxplus_{(0, +\infty)}$, $\boxplus_{[0, +\infty)}$, $\boxminus_{(0, +\infty)}$, $\boxminus_{[0, +\infty )}$ to these metric atoms whose predicates in $A_{invariant}$ unless their interval contain infinite or infinitesimal value.

For metric atoms whose predicates are in $A_{variant}$, one knotty problem is whether their corresponding unbounded metric atoms should be included. To this end, we adopt a heuristic method,
that is, for $\boxplus_{(0, +\infty)}M$, $\boxplus_{[0, +\infty )}M$, we will include them if $M$ always holds from some ruler interval, $\varrho_s$ to $\varrho_{e}$, where $\varrho_{e}$ is the maximum ruler interval where \emph{partial materialisation} terminates; for $\boxminus_{(0, +\infty)}M$, $\boxminus_{[0, +\infty )}M$, we also apply the similar strategy.


==> related_works.tex <==
\section{Related Works}
In the field of Datalog, \emph{Materialisation} has been widely used to improve the performance of systems. More specifically, Datalog-based system usually \emph{materialise} all consequences of a datalog program and the data in a preprocessing step, over which users' queries could be direclty evaluated~\cite{motik2014parallel}.


==> ruler.tex <==
\begin{tikzpicture}[scale=0.75]
%[x=1.05cm,y=1.05cm]

\footnotesize

\tikzset{>=latex}

\draw[<->, thick, gray] (-2,0)--(6,0);

%\node(rho1) at (-2.5,0){ }; 
\node(rho2) at (-0.8,0){ }; 
\node(rho3) at (0,0){ }; 
\node(rho4) at (1.7,0){ };
\node(rho5) at (2.5,0){ };
\node(rho6) at (4.2,0){ }; 
\node(rho7) at (5,0){ };


\node(rho2_up)  at ($(rho2)+(0,0.1)$) {};
\node(rho2_down)  at ($(rho2)+(0,-0.1)$) {};
\draw[-, very thick] (  rho2 |- rho2_up) -- (rho2 |- rho2_down);
\node[below  = 0.01 of rho2] {$-0.8$};

\node(rho3_up)  at ($(rho3)+(0,0.1)$) {};
\node(rho3_down)  at ($(rho3)+(0,-0.1)$) {};
\draw[-, very thick] (  rho3 |- rho3_up) -- (rho3 |- rho3_down);
\node[below  = 0.01 of rho3] {$0$};
%\node[ label={[yshift=-2]{$\alpha$}}] at (rho3) {};

\node(rho4_up)  at ($(rho4)+(0,0.1)$) {};
\node(rho4_down)  at ($(rho4)+(0,-0.1)$) {};
\draw[-, very thick] (  rho4 |- rho4_up) -- (rho4 |- rho4_down);
\node[below  = 0.01 of rho4] {$1.7$};

\node(rho5_up)  at ($(rho5)+(0,0.1)$) {};
\node(rho5_down)  at ($(rho5)+(0,-0.1)$) {};
\draw[-, very thick] (  rho5 |- rho5_up) -- (rho5 |- rho5_down);
\node[below  = 0.01 of rho5] {$2.5$};

\node(rho6_up)  at ($(rho6)+(0,0.1)$) {};
\node(rho6_down)  at ($(rho6)+(0,-0.1)$) {};
\draw[-, very thick] (  rho6 |- rho6_up) -- (rho6 |- rho6_down);
\node[below  = 0.01 of rho6] {$4.2$};
%\node[ label={[yshift=-2]{$\beta$}}] at (rho6) {};

\node(rho7_up)  at ($(rho7)+(0,0.1)$) {};
\node(rho7_down)  at ($(rho7)+(0,-0.1)$) {};
\draw[-, very thick] (  rho7 |- rho7_up) -- (rho7 |- rho7_down);
\node[below  = 0.01 of rho7] {$5$};


\node at ($(rho2)+(0,0.4)$) [circle,fill,inner sep=1pt]{};

\draw[(-), thick] ($(rho2)+(0.1,0.4)$) -- 
($(rho3)+(-0.1,0.4)$);

\node at ($(rho3)+(0,0.4)$) [circle,fill,inner sep=1pt]{};

\draw[(-), thick] ($(rho3)+(0.1,0.4)$) -- 
($(rho4)+(-0.1,0.4)$);

\node at ($(rho4)+(0,0.4)$) [circle,fill,inner sep=1pt]{};

\draw[(-), thick] ($(rho4)+(0.1,0.4)$) -- 
($(rho5)+(-0.1,0.4)$);

\node at ($(rho5)+(0,0.4)$) [circle,fill,inner sep=1pt]{};

\draw[(-), thick] ($(rho5)+(0.1,0.4)$) -- 
($(rho6)+(-0.1,0.4)$);

\node at ($(rho6)+(0,0.4)$) [circle,fill,inner sep=1pt]{};

\draw[(-), thick] ($(rho6)+(0.1,0.4)$) -- 
($(rho7)+(-0.1,0.4)$);

\node at ($(rho7)+(0,0.4)$) [circle,fill,inner sep=1pt]{};



\node[ label={[yshift=-21]{Ruler:}}] at (-4,0.15) {};

\node[ label={[yshift=-13]{ Ruler-intervals:}}] at (-3.2,0.65) {};

\end{tikzpicture}

==> tab/ablation.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{l|c|c|c}
         \hline 
         \hline 
         \multicolumn{2}{c|}{} & $\D_1$($5.42 \cdot 10^6$ facts) &  $\D_2$($7.99 \cdot 10^6$ facts) \\
          \hline 
          \multirow{2}{*}{$M1@\varrho1$} & Ours($\Prog$)  & $0.42$s  &   $0.66$s  \\
          \cline{2-4} 
          & Ours~($\Prog^{M1}$) &  $0.33$s &  $0.46$s\\
          \hline 
           \multirow{2}{*}{$M2@\varrho2$} &  Ours($\Prog$)  &  $0.81$s & $1.56$s  \\
         \cline{2-4} 
          
          & Ours($\Prog^{M2}$) &  $0.59$s  &  $0.93$s  \\
         
          \hline 
         \hline 
    \end{tabular}
    \caption{Results of ablation study }
    \label{tab:ablation}
\end{table}

==> tab/recusive.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{l|c|c}
         \hline 
         \hline 
         & $\D_1$($5.42 \cdot 10^6$ facts) &  $\D_2$($7.99 \cdot 10^6$ facts)  \\
         \hline 
          ($\Prog$, $M^{r}@\varrho1$) &  $0.0021$s &  $0.0025$s \\
          \hline 
          ($\Prog$, $M^{r}@\varrho2$) &  $4.1$s~(25) & $7.4$s~(22)  \\
          \hline 
          ($\Prog$, $M^{r}@\varrho3$) &  $9.13$min &   $30.13$min \\
          \hline 
         \hline 
    \end{tabular}
    \caption{Evaluation of our reasoner on recursive scenarios. Number in the bracket denotes the number of steps of materialisation. Note that for the sake of fairness, the reported time does not include the time for loading $\D$ in our approach and the time for loading $\D$ into the Postgres datatabase in SQL approach. $\Prog$ is the program from Example~\ref{examplegraph}. Predicates of three $M^{r}@\varrho1$, $M^{r}@\varrho2$ and $M^{r}@\varrho3$ are $\textit{FullProfessor}$ but with different intervals.}
    \label{tab:recursive}
\end{table}

==> tab/statistics.tex <==
% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|c|c|c|c}
%          & \# of predicates &
%         $\D_1$ &  \\
%         $\D_2$ &  \\
%         $\D_3$ &  \\
%         $\D_4$ &  \\
        
%     \end{tabular}
%     \caption{Statistics for testing datasets and programs }
%     \label{tab:my_label}
% \end{table}

\begin{table}[]
    \centering
    \begin{tabular}{c|c|c|c|c}
         \hline 
         \multicolumn{5}{c}{\textbf{Datasets}}  \\
         \hline 
         & $\D_1$ &  $\D_2$ &  $\D_3$ &  $\D_4$  \\
         \hline 
         \# of facts ($\times 10^6$) &  5.42 &  7.99 &  13.70 &  27.39 \\
         \hline 
         \hline 
         \multicolumn{5}{c}{\textbf{Programs}}  \\
         \hline 
         \multicolumn{2}{c|}{} & $\Prog_{nr}$ & $\Prog_{nrr}$ & $\Prog_{r}$ \\
         \hline 
         \multicolumn{2}{c|}{$\mathit{\#}$ of rules} & 14 & 0 & 0  \\
         \hline 
         \multicolumn{2}{c|}{\# of non-recursive} & 10 & 15 & 4  \\
         \hline 
         \multicolumn{2}{c|}{\# of recursive} & 10 & 15 & 4  \\
         \hline 
    \end{tabular}
    \caption{Statistics for Datasets and Programs}
    \label{tab:data}
\end{table}
